ZeroI2V: Zero-Cost Adaptation of Pre-trained Transformers from Image to Video

Adapting image models to the video domain has emerged as an efficient paradigm for solving video recognition tasks. Due to the huge number of parameters and effective transferability of image models, performing full fine-tuning is less efficient and even unnecessary. Thus, recent research is shifting its focus toward parameter-efficient image-to-video adaptation. However, these adaptation strategies inevitably introduce extra computational costs to deal with the domain gap and temporal modeling in videos. In this paper, we present a new adaptation paradigm (ZeroI2V) to transfer the image transformers to video recognition tasks (i.e., introduce zero extra cost to the original models during inference). To achieve this goal, we present two core designs. First, to capture the dynamics in videos and reduce the difficulty of image-to-video adaptation, we exploit the flexibility of self-attention and introduce spatial-temporal dual-headed attention (STDHA). This approach efficiently endows the image transformers with temporal modeling capability at zero extra parameters and computation. Second, to handle the domain gap between images and videos, we propose a linear adaption strategy that utilizes lightweight densely placed linear adapters to fully transfer the frozen image models to video recognition. Thanks to the customized linear design, all newly added adapters could be easily merged with the original modules through structural reparameterization after training, enabling zero extra cost during inference. Extensive experiments on representative fully-supervised and few-shot video recognition benchmarks showcase that ZeroI2V can match or even outperform previous state-of-the-art methods while enjoying superior parameter and inference efficiency.

==> tables/sota_diving48.tex <==
\begin{table}[h]
    \centering
    \caption{\textbf{Comparing the state-of-the-art video recognition methods on Diving48.} We test our method with 1 temporal clip following AIM~\cite{yangaim}.}
    \label{tab:diving48}
    \begin{tabular}{lcc}
        \toprule
        Method & Pretrain & Top-1  \\
        \midrule
        \multicolumn{3}{@{}l}{\it Methods with full fine-tuning} \\
        % rgbonly methods \\
        TimeSformer-L~\cite{timesformer} & IN21K & 81.0 \\
        VideoSwin-B~\cite{videoswin} & IN21K & 81.9 \\
        BEVT~\cite{bevt} & IN21K+K400& 87.2 \\
        SIFAR-B ~\cite{sifar} & IN21K & 87.3 \\
        % \midrule
        % additional modalitiy methods \\
        \midrule
        \multicolumn{3}{@{}l}{\it Methods with PETL} \\
        AIM ViT-B/16~\cite{yangaim} & CLIP & 88.9 \\
        AIM ViT-L/14~\cite{yangaim} & CLIP & 90.6 \\
        \midrule
        \textbf{ZeroI2V} ViT-B/16 & CLIP & 89.7 \\
        \textbf{ZeroI2V} ViT-L/14 & CLIP & \textbf{91.4} \\
        \bottomrule
    \end{tabular}
    \label{tab:ucf_hmdb}
\end{table}

==> tables/sota_swin.tex <==
\begin{table}[ht] %[!t]
    \centering
    \caption{\textbf{Results on K400 validation set with Swin-B backbone.} K400\dag/K600\dag indicates that the model is pre-trained on both IN21K and K400/K600. The other notations are the same as Table \ref{tab:sota_in21k}. Views for all methods are 32\(\times\)3\(\times\)4 for K400 and 32\(\times\)3\(\times\)1 for SSv2}
    \tablestyle{4.8pt}{1.1}
    
\begin{tabular}{@{}y{88}x{30}x{30}x{30}x{30}x{30}x{30}x{28}x{28}@{}}
\toprule
Methods & Pretrain  & GFLOPs & Extra GFLOPs  & Param(M) & New Param(M) & K400 Top-1 & SSv2 Top-1 \\
\toprule
\multicolumn{8}{@{}l}{\it Methods with full fine-tuning} \\
VideoSwin-B~\cite{videoswin} & IN21K  & 282 & - & 89 & - &  \textbf{82.7} & -  \\
VideoSwin-B~\cite{videoswin} & K400\dag  & 321 & - & 89 & -  &  - & 69.6  \\
PST Swin-B~\cite{tps} & IN21K & 247 & 0 & 89 & 0 & 81.8 & 67.4 \\
% PST Swin-B~\cite{tps} & K400\dag & 247 & - & 89 & - & - & 69.2 \\
% Swin-T w/ \textbf{STDHA} & IN21K & - & - & 28 & - & - & - \\
Swin-B w/ \textbf{STDHA} & IN21K & 247 & 0 & 89 & 0 & 82.1 & \textbf{70.0} \\
\midrule
\multicolumn{8}{@{}l}{\it Methods with PETL} \\
AIM Swin-B~\cite{yangaim} & IN21K  &  & & 107 & 9   &  82.1   & - \\

\textbf{ZeroI2V} Swin-B & IN21K &  &  &  &    & & 67.8 \\ 
\bottomrule
\end{tabular}

\label{tab:sota_swin}
\end{table}



==> tables/sota_ucf101_hmdb51.tex <==
\begin{table}[h]
    \centering
    \caption{\textbf{Comparing the state-of-the-art video recognition methods on UCF101 and HMDB51.} We test our method and report the 3-split mean Top-1 accuracy for both datasets following ST-Adapter~\cite{stadapter}.}
    \label{tab:ucfhmdb}
    \begin{tabular}{lccc}
        \toprule
        Method & Pretrain & UCF101 & HMDB51 \\
        \midrule
        \multicolumn{4}{@{}l}{\it Methods with full fine-tuning} \\
        % rgbonly methods \\
        STC~\cite{stc} & K400 & 95.8 & 72.6 \\
        % ARTNet \cite{artnet}& & K400 & 94.3 & 70.9 \\
        ECO~\cite{eco} & K400 & 93.6 & 68.4 \\

        I3D~\cite{i3dk400} & ImageNet+K400 & 95.6 & 74.8 \\
        S3D~\cite{s3d} & ImageNet+K400 & 96.8 & 75.9 \\
        SlowOnly-8x8-R101~\cite{slowfast} & Kinetics+OmniSource & 97.3 & 79.0 \\
        VideoPrompt~\cite{videoprompt} & CLIP & 93.6 & 66.4 \\
        % \midrule
        % additional modalitiy methods \\
        \midrule
        \multicolumn{4}{@{}l}{\it Methods with PETL} \\
        ST-Adapter ViT-B/16~\cite{stadapter} & CLIP+K400 & 96.4 & 77.7 \\
        ST-Adapter ViT-L/14~\cite{stadapter} & CLIP+K400 & 98.1 & 81.7 \\
        \midrule
        \textbf{ZeroI2V} ViT-B/16 & CLIP & 95.6 & 73.7 \\
        \textbf{ZeroI2V} ViT-B/16 & CLIP+K400 & 97.7 & 78.5 \\
        \textbf{ZeroI2V} ViT-L/14 & CLIP & 97.8 & 79.9 \\
        \textbf{ZeroI2V} ViT-L/14 & CLIP+K400 & \textbf{98.6} & \textbf{83.4} \\
        \bottomrule
    \end{tabular}
    \label{tab:ucf_hmdb}
\end{table}
